Bandwidth selection for kernel density estimators of multivariate level sets and highest density regions

We consider bandwidth matrix selection for kernel density estimators (KDEs) of density level sets in $\mathbb{R}^d$, $d \ge 2$. We also consider estimation of highest density regions, which differs from estimating level sets in that one specifies the probability content of the set rather than specifying the level directly. This complicates the problem. Bandwidth selection for KDEs is well studied, but the goal of most methods is to minimize a global loss function for the density or its derivatives. The loss we consider here is instead the measure of the symmetric difference of the true set and estimated set. We derive an asymptotic approximation to the corresponding risk. The approximation depends on unknown quantities which can be estimated, and the approximation can then be minimized to yield a choice of bandwidth, which we show in simulations performs well. We provide an R package lsbs for implementing our procedure.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% combined packages and macros preamble.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% %% some of my preamble 'best practices':

%% package xparse allows for 'macro overloading' in a sense but i havent used
%% it yet.

%% natbib, hyperref   used right now ; have caused errors in past

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\usepackage[inline]{enumitem}
% \usepackage{newclude}
\usepackage{versions}
% \usepackage{graphicx}
% \usepackage{times}
%\usepackage{fancyvrb}
% \usepackage{geometry}  %% currently make geometry modifications in each
% specific doc


\usepackage[english]{babel}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{amssymb,dsfont,mathtools}
\usepackage{bbm} %% mathbb vs mathbbm?  I use bbm for indicator fns.
\usepackage{amsthm} %% do i want/ use this correctly?
\usepackage{epsfig, subfigure}
\usepackage{natbib}
\usepackage{color}
\RequirePackage[colorlinks,linkcolor=red,citecolor=blue,urlcolor=blue]{hyperref}
% \RequirePackage{hypernat}

% \usepackage{url}

%% table packages
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{slashbox}

% \usepackage[demo]{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}

\setlength{\textwidth}{5.5in}
\setlength{\textheight}{21cm}

% \pdfoutput=1
% \newcommand{\com}[1]{{\noindent  \color{blue}#1}}       % blue, magenta
% \newcommand{\comC}[1]{{\noindent  \color{magenta}#1}}
\newcommand{\KR}[1]{{\noindent  \color{red}#1}}
\newcommand{\FB}[1]{{\noindent  \color{blue}#1}}

\newcommand{\comf}[1]{{\noindent \color{blue}#1}}
\newcommand{\remf}[1]{{\noindent \color{magenta}#1}}


%% here here

\let\proglang=\textsf
\newcommand{\pkg}[1]{{\fontseries{b}\selectfont #1}}
\let\code=\texttt


\usepackage{xparse} %% multi-optional-arguments in macros.
\usepackage{etoolbox} %% gives 'ifstrempty' command


\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem*{proposition*}{Proposition}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{lemma*}{Lemma}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem*{definition*}{Definition}
\newtheorem*{remark*}{Remark}
\newtheorem*{example*}{Example}
% \newtheorem{assumption}{Assumption}[section] %% constr approx style deals
% % poorly with seciton numbering it seems
%% \newtheorem{assumption}{Assumption}
% \newtheorem{conjecture}{Conjecture}[section]

\newtheorem*{assumption*}{\assumptionnumber}
\providecommand{\assumptionnumber}{}
\makeatletter % changes the catcode of @ to 11 from 12
\newenvironment{assumption}[1]
 {%
  \renewcommand{\assumptionnumber}{Assumption #1}%
  \begin{assumption*}%
  \protected@edef\@currentlabel{#1}%
 }
 {%
  \end{assumption*}
 }
\makeatother % changes the catcode of @ back to 12


%\newcommand{\prf}{\begin{proof}{Proof}}







% --------------------------------------------------------------%
% COMMENTS COLORS

\usepackage[usenames,dvipsnames]{xcolor}

\newcommand{\remC}[1]{{\noindent \color{Green}#1}}


\newcommand{\comC}[1]{{\noindent  \color{Maroon}#1}}       % blue, magenta
% \newcommand{\comJ}[1]{{\noindent   \color{green}#1}}       % blue, magenta
\newcommand{\comF}[1]{{\noindent   \color{Dandelion}#1}}       % blue, magenta
\newcommand{\comOld}[1]{{\noindent  \color{OliveGreen}#1}}       % blue, magenta
% potential colors ( from http://en.wikibooks.org/wiki/LaTeX/Colors):
% Bittersweet, OliveGreen,  BurntOrange, Maroon
% --------------------------------------------------------------%

\usepackage{float}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%% NOTE: xparse provides method to differentiate between no argument and
%% empty argument (IfNoValueTF; use o instead of O{}).  But i'm not using
%% that, don't want it.  In this definition, the arguemnts are sequential, so
%% dont need to test all combinations just for the last one.
% \NewDocumentCommand\testtt{O{}O{}O{}}{
%   \ifstrempty{#1}{
%     N_{[\, ]}
%   }{
%     \ifstrempty{#2}
%     {MISTAKE}
%     {\ifstrempty{#3}{MISTAKE}
%     {N_{[\, ]} \left( {#1}, {#2}, {#3} \right)}}
%   }
% }

% \NewDocumentCommand\Nb{O{}}{
%   \ifstrempty{#1}{
%     N_{[\, ]}
%   }{
%     N_{[\, ]}\left( {#1} \right)
%   }
% }

% \NewDocumentCommand\Nc{O{}}{
%   \ifstrempty{#1}{
%     N
%   }{
%     N\left( {#1} \right)
%   }
% }

% %% just have one argument; typing the commas is easy
% \NewDocumentCommand\cC{O{}}{
%   \ifstrempty{#1}{
%     \mc C
%   }{
%     \mc C \left( {#1} \right)
%   }
% }


\DeclareMathOperator{\vol}{Vol}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\diam}{diam}
\global\long\def\inv#1{\frac{1}{#1}}
\DeclareMathOperator*{\Bias}{Bias}
\DeclareMathOperator*{\MSE}{MSE}
\DeclareMathOperator*{\Var}{Var}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\Cor}{Cor}
\DeclareMathOperator*{\sd}{sd}
% \DeclareMathOperator*{\min}{min}
% \DeclareMathOperator*{\max}{max}
%% \mathrm is owrose than declaremathoperator
%\newcommand{\dom}{\mathrm{dom}}
%\newcommand{\sub}{\mathrm{sub}}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\sub}{sub}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}






















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  Macros below here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\newcommand{\lp}{\left(} %% )
  \newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{} %% )
  \newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[} %% )
  \newcommand{\rs}{\right]}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\lv}{\left\vert}
\newcommand{\rv}{\right\vert}
\newcommand{\lV}{\left\Vert}
\newcommand{\rV}{\right\Vert}
%\newcommand{\|}{\Vert}

\newcommand{\vp}{\varphi}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}


\newcommand{\ve}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\ve{#1}}

%% \newcommand{\cC}{\mathcal{C}} %% see below
\newcommand{\PP}{{\mathbb P}}
\newcommand{\PPn}{{\mathbb P}_n}
\newcommand{\FFn}{{\mathbb F}_n}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\GGn}{{\mathbb G}_n}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{{\mathbb Z}}



\newcommand{\ib}{\boldsymbol{i}}
\newcommand{\jb}{\boldsymbol{j}}
\newcommand{\Gb}{\boldsymbol{\Gamma}}



\newcommand{\eps}{\varepsilon}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\pp}{\ensuremath{\mathfrak{P}}}
% \newcommand{\ff}{\ensuremath{\mathfrak{F}}}
\newcommand{\fft}{\ensuremath{\tilde{\mathfrak{F}}}}
\newcommand{\ffn}{\ensuremath{{\mathfrak{F}}^{\otimes n}}}
\newcommand{\ffb}{\ensuremath{\ff_{\text{BDD}}}}
\newcommand{\ffs}{\ensuremath{\ff_{\text{SMU}}}}


\newcommand{\one}{\mathbbm{1}}
\newcommand{\bb}[1]{\mathbb {#1}}
\newcommand{\kl}[2]{\rho_{\mathrm{KL}}\left({#1} \, \Vert \, {#2} \right)}
\newcommand{\mc}[1]{\mathcal {#1}}
\newcommand{\bs}[1]{\boldsymbol {#1}}

\newcommand{\cI}{\mathcal{I}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bz}{\boldsymbol{z}}

\newcommand{\wh}{\widehat}

% \newcommand{\argmin}{\mathrm{argmin}}
%%\newcommand{\inf}{\mathrm{inf}}
%%\newcommand{\sup}{\mathrm{sup}}
\newcommand{\limsupp}{{\overline{\mathrm{lim}}}}
\newcommand{\ess}{{{\mathrm{ess}}}}
%% \newcommand{\width}{{\mathrm{width}}}
\newcommand{\SPAN}{{\mathrm{span}}}

\newcommand{\adj}{\operatorname{adj}}
\newcommand{\linaff}{\operatorname{Lin}}
%% \newcommand{\lin}{{\mathrm{lin}}}
\newcommand{\Lin}{\operatorname{Lin}}


%% polar coords; just regular font for now?
\NewDocumentCommand\PC{O{}}{
        \ifstrempty{#1}{
        P^{d-1}
        }{
        P^{#1}
        }
}
%% polar coords; just regular font for now?
\NewDocumentCommand\PCc{O{}}{
        \ifstrempty{#1}{
        \overline{P}^{d-1}
        }{
        \overline{P}^{#1}
        }
}

\NewDocumentCommand\ffnH{O{}}{
  \ifstrempty{#1}{
  \widehat{f}_{n,\bH}
  }{
  \widehat{f}_{#1}
  }
}

\NewDocumentCommand\fftaun{O{}}{
  \ifstrempty{#1}{
  \widehat{f}_{\tau, n}
  }{
  \widehat{f}_{\tau, #1}
  }
}
\NewDocumentCommand\fftau{O{}}{
  \ifstrempty{#1}{
       f_{\tau,0}
  }{
        f_{\tau,#1}
  }
}

\NewDocumentCommand\LLtau{O{}}{
  \ifstrempty{#1}{
  L
  }{
   L_{#1}
  }
}
\NewDocumentCommand\deriv{m O{}}{
  \ifstrempty{#2}{
  \frac{d}{d #1}
  }{
  \frac{d #2}{d #1}
  }
}

\NewDocumentCommand\pderiv{m O{}}{
  \ifstrempty{#2}{
  \frac{\partial}{\partial #1}
  }{
  \frac{\partial #2}{\partial #1}
  }
}
\NewDocumentCommand\derivtwo{m m O{}}{
  \ifstrempty{#3}{
  \frac{\partial^2}{\partial #1 \partial #2}
  }{
  \frac{\partial^2 #3}{\partial #1 \partial #2}
  }
}



\DeclareMathOperator{\LS}{LS}
\DeclareMathOperator{\HDR}{HDR}

\newcommand{\bracketing}{N_{[\,]}} %% deprecated
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}}
\newcommand{\ind}{\stackrel{\text{ind}}{\sim}}





\newenvironment{solution}{%
  \par \vspace{.2cm} { \bf Solution:}%
}{%
  \vspace{.2cm}
}

% \newenvironment{longform}{%
%   \par \vspace{.2cm} { \bf (Begin) Notes to self:}%
% }{%
%         \bf (End) Notes to self:  \vspace{.2cm}
% }
\newenvironment{longform}{%
        \color{gray}
}{\ignorespacesafterend}


%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: "p"
%%% End:

